The Dark Energy Survey Image Processing Pipeline

The Dark Energy Survey (DES) is a five-year optical imaging campaign with the goal of understanding the origin of cosmic acceleration. DES performs a 5000 square degree survey of the southern sky in five optical bands (g,r,i,z,Y) to a depth of ~24th magnitude. Contemporaneously, DES performs a deep, time-domain survey in four optical bands (g,r,i,z) over 27 square degrees. DES exposures are processed nightly with an evolving data reduction pipeline and evaluated for image quality to determine if they need to be retaken. Difference imaging and transient source detection are also performed in the time domain component nightly. On a bi-annual basis, DES exposures are reprocessed with a refined pipeline and coadded to maximize imaging depth. Here we describe the DES image processing pipeline in support of DES science, as a reference for users of archival DES data, and as a guide for future astronomical surveys.

==> data/yanny_authors.tex <==
\author{Eric Morganson\altaffilmark{1,2}}
\author{Robert A. Gruendl\altaffilmark{1,2}}
\author{Felipe Menanteau\altaffilmark{1,2}}

%\author{Emmanuel Bertin\altaffilmark{XX}}
\author{Matias Carrasco Kind\altaffilmark{1,2}}
\author{Yu-Ching Chen\altaffilmark{1,2}}
\author{Greg Daues\altaffilmark{1,2}}
\author{Douglas N. Friedel\altaffilmark{1,2}}
\author{Michelle Gower\altaffilmark{1,2}}
\author{Margaret Johnson\altaffilmark{1,2}}
\author{Michael Johnson\altaffilmark{1,2}}
\author{Richard Kessler\altaffilmark{3,4}}
%\author{John Marriner\altaffilmark{5}}
\author{Francisco Paz-Chinch\'on\altaffilmark{1,2}}
\author{Don Petravick\altaffilmark{1,2}}
\author{Chris Pond\altaffilmark{1,2}}
%\author{Ignacio Sevillai\altaffilmark{XX}}
%\author{Douglas Tucker\altaffilmark{5}}
\author{Brian Yanny\altaffilmark{5}}
\author{Sahar Allam\altaffilmark{5}}
\author{Bob Armstrong\altaffilmark{6}}
\author{Wayne Barkhouse\altaffilmark{7}}
\author{Aur{\'e}lien Benoit-L{\'e}vy\altaffilmark{8,9,10}}
\author{Gary Bernstein\altaffilmark{11}}
\author{Emmanuel Bertin\altaffilmark{8,10}}
\author{Elizabeth Buckley-Geer\altaffilmark{5}}
\author{Shantanu Desai\altaffilmark{12}}
\author{H. Thomas Diehl\altaffilmark{5}}
\author{Alex Drlica-Wagner\altaffilmark{5}}
\author{Daniel Goldstein\altaffilmark{13}}
\author{Daniel Gruen\altaffilmark{14,15}}
\author{Huan Lin\altaffilmark{5}}
\author{John Marriner\altaffilmark{5}}
\author{Joe Mohr\altaffilmark{16,17,18}}
\author{Eric Neilsen\altaffilmark{5}}
\author{Chow-Choong Ngeow\altaffilmark{19}}
\author{Kerstin Paech\altaffilmark{16,20}}
\author{Eli Rykoff\altaffilmark{14,15}}
\author{Masao Sako\altaffilmark{11}}
\author{Ignacio Sevilla\altaffilmark{21}}
\author{Erin Sheldon\altaffilmark{22}}
\author{Flavia Sobreira\altaffilmark{23,24}}
\author{Douglas Tucker\altaffilmark{5}}
\author{William Wester\altaffilmark{5}}

\affil{$^1$National Center for Supercomputing Applications,University of Illinois at Urbana-Champaign 1205 W. Clark St., Urbana, IL 61801}
\affil{$^2$Department of Astronomy,University of Illinois at Urbana-Champaign 1002 W. Green Street, Urbana, IL 61801}
%\affil{$^XX$Institut d'Astrophysique, 98bis, bd Arago, Paris, France 75014;}
\affil{$^3$Kavli Institute for Cosmological Physics, University of Chicago, Chicago, IL 60637, USA}
\affil{$^4$Department of Astronomy and Astrophysics, University of Chicago, 5640 South Ellis Avenue, Chicago, IL 60637, USA}
\affil{$^5$Fermi National Accelerator Laboratory, P. O. Box 500, Batavia, IL, USA 60510}
%\affil{$^XX$Centro de Investigaciones Energeticas Medioambiantales y Tocnologicas, Av. Complutense 40, Madrid, SP 28040}
\affil{$^6$Department of Astrophysical Sciences, Princeton University, Peyton Hall, Princeton, NJ 08544, USA}
\affil{$^7$University of North Dakota, Department of Physics and Astrophysics, Witmer Hall, Grand Forks, ND 58202, USA}
\affil{$^8$CNRS, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
\affil{$^9$Department of Physics \& Astronomy, University College London, Gower Street, London, WC1E 6BT, UK}
\affil{$^{10}$Sorbonne Universit\'es, UPMC Univ Paris 06, UMR 7095, Institut d'Astrophysique de Paris, F-75014, Paris, France}
\affil{$^{11}$Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104, USA}
\affil{$^{12}$Department of Physics, IIT Hyderabad, Kandi, Telangana 502285, India}
\affil{$^{13}$Department of Astronomy, University of California, Berkeley,  501 Campbell Hall, Berkeley, CA 94720, USA}
\affil{$^{14}$Kavli Institute for Particle Astrophysics \& Cosmology, P. O. Box 2450, Stanford University, Stanford, CA 94305, USA}
\affil{$^{15}$SLAC National Accelerator Laboratory, Menlo Park, CA 94025, USA}
\affil{$^{16}$Excellence Cluster Universe, Boltzmannstr.\ 2, 85748 Garching, Germany}
\affil{$^{17}$Faculty of Physics, Ludwig-Maximilians-Universit\"at, Scheinerstr. 1, 81679 Munich, Germany}
\affil{$^{18}$Max Planck Institute for Extraterrestrial Physics, Giessenbachstrasse, 85748 Garching, Germany}
\affil{$^{19}$Graduate Institute of Astronomy, National Central University, Jhongli 32001, Taiwan; ORCID: 0000-0001-8771-7554}
\affil{$^{20}$Universit\"ats-Sternwarte, Fakult\"at f\"ur Physik, Ludwig-Maximilians Universit\"at M\"unchen, Scheinerstr. 1, 81679 M\"unchen, Germany}
\affil{$^{21}$Centro de Investigaciones Energ\'eticas, Medioambientales y Tecnol\'ogicas (CIEMAT), Madrid, Spain}
\affil{$^{22}$Brookhaven National Laboratory, Bldg 510, Upton, NY 11973, USA}
\affil{$^{23}$Instituto de F\'isica Gleb Wataghin, Universidade Estadual de Campinas, 13083-859, Campinas, SP, Brazil}
\affil{$^{24}$Laborat\'orio Interinstitucional de e-Astronomia - LIneA, Rua Gal. Jos\'e Cristino 77, Rio de Janeiro, RJ - 20921-400, Brazil}


==> sources/sources.tex <==
\section{Object Detection and catalogs}


